Proactive Multi-Camera Collaboration For 3D Human Pose Estimation

This paper presents a multi-agent reinforcement learning (MARL) scheme for proactive Multi-Camera Collaboration in 3D Human Pose Estimation in dynamic human crowds. Traditional fixed-viewpoint multi-camera solutions for human motion capture (MoCap) are limited in capture space and susceptible to dynamic occlusions. Active camera approaches proactively control camera poses to find optimal viewpoints for 3D reconstruction. However, current methods still face challenges with credit assignment and environment dynamics. To address these issues, our proposed method introduces a novel Collaborative Triangulation Contribution Reward (CTCR) that improves convergence and alleviates multi-agent credit assignment issues resulting from using 3D reconstruction accuracy as the shared reward. Additionally, we jointly train our model with multiple world dynamics learning tasks to better capture environment dynamics and encourage anticipatory behaviors for occlusion avoidance. We evaluate our proposed method in four photo-realistic UE4 environments to ensure validity and generalizability. Empirical results show that our method outperforms fixed and active baselines in various scenarios with different numbers of cameras and humans.

==> sections/archived/introduction_archived.tex <==
\newcommand{\mytriangle}[1]{\tikz{\node[draw=#1,fill=#1,isosceles
triangle,isosceles triangle stretches,shape border rotate=45,minimum
width=0.2cm,minimum height=0.2cm,inner sep=0pt,rotate=180] at (0,0) {};}}
\definecolor{targettrianglecolor}{RGB}{0,255,255}

\vspace{-0.5cm}
\section{Introduction}
\vspace{-0.25cm}

\newcommand{\rulesep}{\unskip\ \vrule\ }
\begin{figure}[b]
\vspace{-10pt}
  \captionsetup[subfigure]{justification=centering}
  \centering
    \begin{subfigure}[c]{0.30\textwidth}
      \includegraphics[width=\textwidth]{iclr2023/figures/intro/1.PNG}
     \caption{Dynamic occlusions lead to failed reconstruction}\label{fig:first_fig_a}
    \end{subfigure} \
    \hfill
    \begin{subfigure}[c]{0.30\textwidth}
      \includegraphics[width=\textwidth]{iclr2023/figures/intro/2.PNG}
      \caption{Constrained MoCap area}\label{fig:first_fig_b}
    \end{subfigure} \
    \rulesep
    \hfill
    \begin{subfigure}[c]{0.325\textwidth}
      \includegraphics[width=\textwidth]{iclr2023/figures/intro/active3dpose_poster.png}
     \caption*{Active MoCap in the wild}\label{fig:first_fig_c}
    \end{subfigure} \
    % \hfill
    \label{fig:scene_with_mesh}
  \caption{
  \textbf{Left}: Two critical challenges in fixed camera approaches.
  \textbf{Right}: Three active cameras collaborate to best reconstruct the 3D pose of the target (marked in \protect\mytriangle{targettrianglecolor}).} 
\end{figure}

Marker-less motion capture (MoCap) has broad commercial applications in many areas such as cinematography, medical research, virtual reality (VR), sports, and {\etc} %.
Their successes can be partly attributed to recent developments in 3D Human pose estimation (HPE) techniques ~\citep{tu2020voxelpose, iskakov2019learnable, qiu2019cross, jafarian2018monet, pavlakos2017harvesting, dong2019fast, lin2021multi}. 
% Why multi-views
% 3D HPE with monocular images and videos is prone to occlusions and depth ambiguities \cite{ma2021context}. In comparison, the multi-views approach leverages the additional views for more depth information to alleviate the occlusion problems \cite{ma2021context}.
% Why active? 
A straightforward implementation to solve multi-views 3D HPE is to use fixed cameras. Although being a convenient solution, it is less effective against dynamic occlusions. Moreover, fixed camera solutions confine tracking targets within a constrained space, therefore less applicable to outdoor MoCap. On the contrary, active cameras such as ones mounted on drones can maneuver proactively against incoming occlusions. Owing to its remarkable flexibility, the active approach has thus attracted overwhelming interest \citep{tallamraju2020aircaprl, ho20213d, nageli2018flycon, xu2017flycap, kiciroglu2019activemocap, zhou2018human, saini2022airpose, cheng2018ihuman3d, Zhang2021-lj}.


Previous works have demonstrated the effectiveness of using active cameras for 3D HPE on a single target in indoor \citep{kiciroglu2019activemocap, cheng2018ihuman3d}, clean landscapes \citep{tallamraju2020aircaprl, nageli2018flycon, zhou2018human, saini2022airpose} or landscapes with scattered static obstacles \citep{ho20213d}.
However, to our best knowledge, we have not seen any existing work that experimented with \emph{multiple} $(n > 3)$ active cameras to conduct 3D HPE \emph{in human crowd}. There are two key challenges : 
\textbf{First}, frequent human-to-human interactions lead to \textbf{random dynamic occlusions}. Different from previous works that only consider clean landscapes or static obstacles, dynamic scenes require frequent adjustments of cameras' viewpoints for occlusion avoidance while keeping an overall good team formation for multi-view reconstruction. Therefore, it is challenging to achieve optimality with a fixed camera formation or a hand-crafted control policy. In addition, the complex behavioral pattern of a human crowd makes the occlusion patterns less comprehensible and predictable, further increasing the difficulty in control. 
\textbf{Second}, as the size of a camera team grows, the \textbf{multi-agent credit assignment issue} becomes prominent which hinders policy learning of the camera agents. Concretely, as a team effort, multi-view 3D HPE requires inputs from multiple cameras to generate an accurate reconstruction. Having more camera agents participate in a reconstruction introduces more redundancy. Though it reduces the susceptibility to reconstruction failure caused by dynamic occlusions, it consequently weakens the association between the individual performance and the reconstruction accuracy of the team, which likely leads to the ``lazy agent'' problem~\citep{vdn2018}. A shared reward risks disincentivizing some individual cameras on exploring better viewpoints due to an adequate accuracy already being attained by their teammates alone.

% Therefore motivated by the Shapley value~\citep{rapoport2001n}, which is a solution concept regarding fair allocation of payouts in cooperative game theory, we proposed the Collaborative Triangulation Contribution Reward (CTCR) that computes the weighted marginal contribution to the 3D reconstruction for any given agent over all possible formations that contain it. This reward aims to correctly associate agents' levels of participation with their actual contributions to the 3D reconstruction and guide their policy learning when the shared team reward alone is insufficient to produce that association.

% of each camera' viewpoint to avoid occlusion of the target while keeping an overall good formation
% where dynamic occlusion is a predominant and non-negligible factor of disturbance. 3D HPE in a human crowd has two challenging aspects:

% First, the behavioral pattern of a crowd are less comprehensible and less predictable due to partial observability of the camera agents. As the camera controllers do not have access to the internal states of humans, they have no prior information on their planned trajectories and destinations.
% Second, dynamic scenes require frequent adjustments relative to the position of the target across multiple views. Due to dynamic occlusions, maintaining a fixed formation for the cameras may not be optimal. 

%As 3D HPE rely on depth information sampled from numerous perspectives, loss of target due to occlusions in one view may lead to complete failure in pose reconstruction. 

% \textbf{Third}, for decentralized control,  It is increasing difficult to assign credit to each of 
% Why crowds? 
% First, in realistic settings cameras have partial observability over the environment, which results in incomplete information about all human locations in the crowd. This will lead to unexpected occlusions, e.g., a previously out-of-sight person could suddenly enter the camera's vision and partially or entirely block its view. Particularly in setups where the number of total views is constrained, loss of one view could lead to failure in pose reconstruction. Second, 
% Why multi-agent
% Decentralized system offers greater flexibility and scalability, also reduces the communication overhead resulted from centralized execution. However, a fully decentralized system is hard to realize due to ...

We introduce a proactive multi-camera collaboration framework based on multi-agent reinforcement learning (MARL) for real-time distributive adjustments of multi-camera formation for 3D HPE in a human crowd.
In our approach, multiple camera agents perform seamless collaboration for successful reconstructions of 3D human poses. 
Additionally, it is a decentralized framework which offers flexibility over the size of formation and eliminates dependency to a control hierarchy or a centralized entity.
% However, the empirical study of the baseline models shows that the off-the-shelf MARL methods perform poorly in such highly dynamic environments. 
In regards of the \textbf{first} challenge, we argue the utmost importance of the model's capability to anticipate human motions and future states of the environment. 
To model these properties in the state representation, we further incorporate \emph{World Dynamics Learning}, i.e., learning with five auxiliary tasks: xxx, xxx, xxx,.
% inspired by \emph{the World Model}~\citep{Ha2018-tu}, 
% Hence, we further incorporate \emph{World Dynamics Learning}, five auxiliary tasks into training to model the dynamics of the environment.
% In this work, we aim to learn multi-camera collaborating strategies for the 3D HPE in human crowd via multi-agent reinforcement learning. A successful reconstruction of 3D human poses requires seamless collaboration between multiple views. Therefore multi-view 3D HPE naturally fits the setting of a collaborative multi-agent reinforcement learning task. Specifically, individual cameras should adjust their positions to where the mean position error of reconstructed poses is minimal.  
% Here, cameras are restricted to local vision, \ie partial observability over the environment, to ensure real-life applicability. 
% We also adapted the \textit{Centralized-Training-Decentralized-Execution} (CTDE) framework to learn a decentralized control policy.
% Although dynamic occlusions present a formidable challenge to accurate 3D HPE, one must tackle the occlusion issues nonetheless since they inherently exist in many real-life applications. Solutions without considering occlusions would be significantly limited in use cases. Therefore in this work, we simulated the crowds with dynamic behaviors such that occlusions are frequent and inevitable if the cameras do not promptly prevent them. The governing module for human actions in our simulation will ensure a diverse generation of trajectories. The simulated human crowd also abides by social norms. For example, yielding right-of-way and collision avoidance. These features mirror the authentic behavioral patterns that resemble a real human crowd, but consequently, more frequent occlusions will take in additional complexities and uncertainties to the 3D HPE task.
% However as shown by our results of the baseline models, the off-the-shelf MARL methods perform poorly in such highly-dynamic environments. 
% We argue the utmost importance of the model's capability to predict human motions and states of the environment. 
% Hence inspired by \textit{the World Model}~\citep{Ha2018-tu}, we incorporate five additional optimization objectives into the training that encourages learning the dynamics of the environment. 
% Concretely, we jointly train Mixture Density Networks (MDNs) \citep{astonpr373} downstream of the feature encoder to predict the future states of the target, pedestrians (non-target humans) and other camera agents. Moreover, we trained MDNs for forward dynamics modelling of own (camera agent) states and rewards.
To tackle the \textbf{second} challenge, we further introduce the \emph{Collaborative Triangulation Contribution Reward (CTCR)}, which incentivizes each agent according to its characteristic contribution to the 3D reconstruction. Inspired by the Shapley Value~\citep{rapoport2001n}, CTCR computes the average weighted marginal contribution to the 3D reconstruction for any given agent over all possible coalitions that contain it. This reward aims to directly associate agents' levels of participation with their return and guides their policy learning when the team reward alone is insufficient to produce such direct association. As a plus, CTCR penalizes occluded camera agents based on individual optimality, encouraging emergent occlusion avoidance behaviors. Empirical results show that CTCR can accelerate convergence and increase reconstruction accuracy. Furthermore, CTCR is a general approach that can benefit policy learning in active 3D HPE and serve as a new assessment metric for view selection in other multi-view reconstruction tasks.


% While further exploring into multi-camera collaboration, we identify the increased difficulty in multi-agent credit assignment with the increasing number of cameras, which leads to early convergence to local minima. 
% As a team effort, 3D HPE with RGB cameras requires inputs from multiple views to generate an accurate reconstruction. Having more camera agents participated in a reconstruction introduces more redundancy. Though the redundancy reduces the susceptibility to reconstruction failure caused by dynamic occlusions, it consequently weakens the association between the individual performance and the reconstruction accuracy, which likely leads to the "lazy" agent problem.
% Therefore motivated by the Shapley value~\citep{rapoport2001n}, which is a solution concept regarding fair allocation of payouts in cooperative game theory, we proposed the Collaborative Triangulation Contribution Reward (CTCR) that computes the weighted marginal contribution to the 3D reconstruction for any given agent over all possible formations that contain it. This reward aims to correctly associate agents' levels of participation with their actual contributions to the 3D reconstruction and guide their policy learning when the shared team reward alone is insufficient to produce that association.


% 3D MoCap in dynamic crowds is a meaningful topic of study with much real-life significance.
% Yet based on our knowledge, we do not notice any publicly available simulation that can service this task without substantial modifications.
% To name a few interesting future directions: MoCap on a film's protagonist during intense action scenes or at a busy pedestrian joint, MoCap of primate crowds in the wild to understand their sociology, real-time 3D biomechanical analysis of athletes in crowded sports events such as Tour De France. 
In experiments, we build photo-realistic environments based on Unreal Engine 4~\citep{UE4} and UnrealCV~\citep{qiu2017unrealcv} for training and testing. Our environments can simulate realistic-behaving crowds with assurances of high fidelity and customizability. We train the agents on a \emph{Blank} environment and validate the generalizability on three unseen test scenes with different landscapes, levels of illumination, human appearances, and various quantities of cameras and humans. The empirical results show that our method can achieve more accurate and stable 3D pose estimates than off-the-shelf passive- and active-camera baselines. To help facilitate more fruitful research on this topic, we will open-source our environments that are integrated with OpenAI Gym-API~\citep{brockman2016openai} and together with a dedicated visualization tool. We summarize the key contributions and demos of this work at the project website\footnote{ \url{https://sites.google.com/view/active3dpose/home}}:

% develop and planned to open-source a toolbox consisting of \textbf{(1)} a virtual environment built with Unreal Engine 4 (UE4) \cite{UE4} that simulates realistic-behaving crowds


% Therefore to help facilitate more fruitful research on this topic, we developed and planned to open-source a toolbox consisting of \textbf{(1)} a virtual environment built with Unreal Engine 4 (UE4) \cite{UE4} that simulates realistic-behaving crowds, \textbf{(2)} a visualization software developed to service frame-by-frame analysis of agents' learned policies, and \textbf{(3)} Python and OpenAI Gym-API \cite{brockman2016openai} integration to support further MARL research regarding active 3D HPE in crowds. 
% The environment allows for high customizability on the landscape, crowd behaviors, and human appearances.

\begin{itemize}[leftmargin=2em]
\vspace{-5pt}
\setlength\itemsep{-0.0em}
    \item We explore the novel problem of active 3D HPE in a human crowd. This work is the first to apply MARL to solve multi-camera collaboration with various quantities of cameras and humans.
    \item We propose CTCR to improve credit assignment in multi-camera collaboration and demonstrate notable improvements in reconstruction accuracy compared to the baselines.
    \item We introduce five auxiliary tasks to help the model learn environment dynamics, further enhancing the model's ability to handle highly dynamic scenes.
    \item We contribute high-fidelity environments built for simulating realistic-looking human crowds with authentic behaviors, along with visualization software for frame-by-frame video analysis.
\end{itemize}




==> sections/old_abstract.tex <==
\begin{abstract}
% \textcolor{red}{per the format requirement: citation number should be in the ascent order like [1], [2],[5]. Adjust this when we are about to finish writing.}
% The abstract should summarize the contents of the paper. LNCS guidelines
% indicate it should be at least 70 and at most 150 words. It should be set in 9-point
% font size and should be inset 1.0~cm from the right and left margins.
% \dots
% 3D Human Pose Estimation (HPE) in crowds remains a formidable challenge, mainly due to the uncertainties incurred from dynamic occlusions. These uncertainties exist due to limited perceptions of the aerial cameras over the environment and varying motion patterns of the pedestrians.


% Motivation
% For, actively-controlled cameras are favored due to their flexibility and scalability over the conventional approaches that rely on fixed or passive cameras. 
% cover a large area, suitable viewpoint (avoid occlusion)


In 3D Human Pose Estimation (HPE), an active camera network can autonomously adjust viewpoint relative to the position of the target to minimize the reconstruction error.
% Proactive cameras mounted on UAVs or rotors can autonomously move and rotate in 3D space to find optimal viewpoints for 3D reconstruction.
This flexibility enables active resolution of occlusions and offers remarkable potential in outdoor mocap applications, \eg, sports assessment. 
% However, it is challenging to realize a distributed multi-camera collaboration scheme due to high dimensionalities, dynamic environment, and noisy reward.
% However, realizing a robust decentralized control policy is challenging as it requires seamless coordination across multiple views on separate entities.
% Briefly describe our work
% In this work, we explored the problem of 3D HPE in crowds through the Unreal Engine 4 simulation environment developed in-house. 
This work aims to develop a proactive multi-camera collaboration scheme for 3D human pose estimation (HPE) in crowds based on multi-agent reinforcement learning (MARL).
% We applied multi-agent reinforcement learning (MARL) to realize proactive, decentralized and occlusion-aware control policies on multiple aerial cameras against crowds with various amounts of people.

% First contribution
To better capture the complex dynamics of the environment, we jointly train the state encoder with multiple world-dynamics learning objectives.

% Empirical results demonstrate a higher reconstruction accuracy in comparison with passive-cameras or active-cameras baselines.
% Second contribution
With the increasing number of cameras ($n > 2$), we further observed the increased prominence of multi-agent credit assignment issue.
Hence, we propose Collaborative Triangulation Contribution Reward (CTCR), a reward function motivated by Shapley Value to incentivize agents based on their actual contributions to the 3D reconstruction.
To ensure validity and generalizability, we evaluate our proposed method on four photo-realistic environments. The empirical results show that our methods steadily outperform the baselines in different scenes with various numbers of cameras and humans.
% that can be configured with different scenes and varying numbers of cameras and humans.
We will open-source our UE4 environments along with a 3D HPE visualization toolkit to facilitate further research in this field.


% We also developed a dedicated visualization software for in-depth qualitative analysis.

\textcolor{red}{Due to high dimensionality of world dynamics and action space, how to find the optimal control policy is intrinsically challenging and remains unclear. put in introduction}

\textcolor{green}{this reward can benefit not only 3D human pose estimation, but also any multi-view 3D reconstruction tasks for efficient view assessment}


\end{abstract}

==> sections/reproducibility.tex <==
\section{Reproducibility Statement}
We will publicly release the project upon the official publishing of this work. The release will include the \textsc{UnrealPose} environment, \textsc{RLlib} training scripts, and the visualization tool. The UE4 binaries and the pre-trained models used in our experiments will also be available for download. The \textsc{RLlib} library is specifically chosen as the base architecture of the implementation of our MARL algorithm. This is to ensure cross-platform compatibility, scalability, maintainability, and transparency.


